Web of Scholars: A Scholar Knowledge Graph

In this work, we demonstrate a novel system, namely Web of Scholars, which integrates state-of-the-art mining techniques to search, mine, and visualize complex networks behind scholars in the field of Computer Science. Relying on the knowledge graph, it provides services for fast, accurate, and intelligent semantic querying as well as powerful recommendations. In addition, in order to realize information sharing, it provides an open API to be served as the underlying architecture for advanced functions. Web of Scholars takes advantage of knowledge graph, which means that it will be able to access more knowledge if more search exist. It can be served as a useful and interoperable tool for scholars to conduct in-depth analysis within Science of Science.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-authordraft.tex \
	samples/sample-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/sample-acmsmall.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmsmall]{acmart}/' $< > $@

samples/sample-acmlarge.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmlarge,screen]{acmart}/' $< > $@

samples/sample-acmtog.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmtog]{acmart}/' $<   > $@

samples/sample-sigconf.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-authordraft.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf,authordraft]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-xelatex.tex: samples/sample-sigconf.tex
	cp $< $@

samples/sample-sigplan.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigplan,screen]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi-a.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi-a]{acmart}/' $< | \
	sed 's/begin{figure}\[h\]/begin{marginfigure}/' | \
	sed 's/end{figure}/end{marginfigure}/' | \
	sed 's/begin{table}/begin{margintable}/' | \
	sed 's/end{table}/end{margintable}/'   > $@


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean


#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst

